Federated Learning based Hierarchical 3D Indoor Localization

The proliferation of connected devices in indoor environments opens the floor to a myriad of indoor applications with positioning services as key enablers. However, as privacy issues and resource constraints arise, it becomes more challenging to design accurate positioning systems as required by most applications. To overcome the latter challenges, we present in this paper, a federated learning (FL) framework for hierarchical 3D indoor localization using a deep neural network. Indeed, we firstly shed light on the prominence of exploiting the hierarchy between floors and buildings in a multi-building and multi-floor indoor environment. Then, we propose an FL framework to train the designed hierarchical model. The performance evaluation shows that by adopting a hierarchical learning scheme, we can improve the localization accuracy by up to 24.06% compared to the non-hierarchical approach. We also obtain a building and floor prediction accuracy of 99.90% and 94.87% respectively. With the proposed FL framework, we can achieve a near-performance characteristic as of the central training with an increase of only 7.69% in the localization error. Moreover, the conducted scalability study reveals that the FL system accuracy is improved when more devices join the training.

==> section/related-work.tex <==
\section{Related work}
\label{sec:related-work}
The related works can be split into two separate aspects namely fingerprinting based DNN localization and federated learning approaches for localization.

In terms of DNN works, the authors in \cite{scalableDNNLocIndoor2017} have presented two distinct architectures for multi-floor, multi-building  and location prediction using WiFi RSSI fingerprinting. 
For the first scheme, they have proceeded in a way that the DNN predicts the logits of the building first, then another inner DNN model is built on top of each output logit to predict the floor. The same process is applied to the floor logits to predict the location which is grid based. Clearly, this approach grows exponentially as the number of building and floor increase as well as the number of grids for the location classification, leading to very complex model difficultly trainable by IoT devices with resources constraints.
Given the limitations of the first approach,  the authors of \cite{scalableDNNLocIndoor2017} have focused on a light weight version of the first approach using a multi-label (building/floor/location) classification. Indeed, the model takes the RSSI as inputs and outputs separately the buildings, the floors, and the location identifiers(ID). The real locations are obtained using a centroid method on the locations sharing the same IDs.  The model global output dimension is thus reduced to the sum of the respective dimensions of the individual outputs, reducing the model complexity even if it introduces a post-processing complexity to obtain the final position. 
Similarly, In \cite{DNNhybrid2018}, the authors have presented a  hybrid   building/floor classification and floor-level 2D location coordinates regression  using  a  single-input  and  multi-output DNN after denoising the RSSI fingerprints with a stacked auto-encoder.  
%###############################
The authors in \cite{CNNLoc3models2019} have seen the indoor positioning as three independent tasks and accordingly, they design three 1D-CNNs models for building, floor, and location classification which is grid based. They achieve 100\% of building prediction accuracy and 95\% success rate on floor-level prediction while the location error is related to the used grid size since the center of the grid is taken as the final location when a device is classified to belong to that grid. Despite these important success rates of building and floor predictions, the approach is very heavy and most of IoT devices cannot support such computation load or may lack memory to store all the models, making their approach impractical.
Recently, \cite{RNNhierachical2021} have proposed a hierarchical  multi-building and  multi-floor  indoor  localization  based  on  a  recurrent  neural network (RNN), eliminating the need of complicated data pre/post-processing and with less parameter tuning. Similarly, \cite{auxiliary2022} have proposed a new framework called a hierarchical auxiliary DNN(HADNN) by inserting classification tasks as auxiliary networks into a regression neural network, so that building, floor and location coordinates are predicted at the same time.
Note that all the aforementioned methods rely on the central training of the models assuming the data availability on the server which is also assumed to be trustworthy. This may lead to issues in practical considerations where data are distributed across IoT devices in a privacy preserving objective. 

%###############################
In the other hand, FL is becoming more attractive for localization problem with its great advantage of privacy by default and the bandwidth saving, especially in wireless communications involving resources constrained IoT devices. In \cite{FedLoc2020}, the authors have shown the prominence of using such algorithm for indoor localization but to date, only a few research works have really tackle the problem. 
Alternatively, the authors in \cite{Etiabi2022FederatedDB} have attempted to solve the indoor localization problem leveraging a more communication friendly FL scenario called \textit{federated distillation} where only
the model outputs whose dimensions are commonly much smaller than the model size are exchanged.
% Finally, Coming to the FD, although FD has been investigated in a bunch of works, only the work presented in \cite{Etiabi2022FederatedDB} has attempted to solve the localization problem leveraging this approach. 
Although, the proposed method was only restricted to location estimation and no information about neither the building nor the floor was provided.

The purpose of this work is to firstly design a DNN architecture for hierarchical 3D localization in multi-building and multi-floor indoor environment, and then investigate a FL scheme to collaboratively train the proposed model.



